Dataset Condensation with Gradient Matching

As the state-of-the-art machine learning methods in many fields rely on larger datasets, storing datasets and training models on them become significantly more expensive. This paper proposes a training set synthesis technique for data-efficient learning, called Dataset Condensation, that learns to condense large dataset into a small set of informative synthetic samples for training deep neural networks from scratch. We formulate this goal as a gradient matching problem between the gradients of deep neural network weights that are trained on the original and our synthetic data. We rigorously evaluate its performance in several computer vision benchmarks and demonstrate that it significantly outperforms the state-of-the-art methods. Finally we explore the use of our method in continual learning and neural architecture search and report promising gains when limited memory and computations are available.

==> relwork.tex <==
\label{sec.relwork}

\paragraph{Coreset selection, continual learning, instance selection.}
% \label{sec:relworks_coreset} 
One of the classical techniques in reducing the size of a large set of high-dimensional points to a small set such that the reduced set approximately preserves a target property (\eg width, diameter) in the original set is coreset selection \cite{agarwal2004approximating,har2004coresets,feldman2013turning}.
Recent examples of this technique can be found in active learning~\cite{sener2017active} and continual learning~\cite{rebuffi2017icarl,toneva2018empirical,castro2018end,aljundi2019gradient}.
Sener and Savarese~\cite{sener2017active} propose an active learning method that picks data points to label from a large set for a fixed labeling budget by using a greedy K-center technique.
In continual learning, coreset selection techniques are commonly used to store a small set of representative samples in a fixed memory budget which is known as replay memory.
Rebuffi~\etal~\cite{rebuffi2017icarl} and Castro~\etal~\cite{castro2018end}
use the herding selection strategy in \cite{welling2009herding} that subsamples the closest samples to the class mean in a feature space. 
Aljundi~\etal~\cite{aljundi2019gradient} cast sample selection as a constraint reduction problem and propose to select a diverse set of samples based on the similarity between their gradients.
Toneva~\etal~\cite{toneva2018empirical} study the relation between the sample selection and forgetability, rate of misclassification during training, and show that the least forgetten samples, a significant fraction of training set can be omitted while still maintaining good performance.
Olvera-López~\etal \cite{olvera2010review} present a review of instance selection methods which aim to reduce the training time by dropping the samples that are not useful for further training. Most of these methods are based on misclassification \cite{hart1968condensed, chou2006generalized} or clustering \cite{mollineda2002efficient, olvera2007restricted}. 

\paragraph{Image synthesis.}
% \label{sec:relatedwork_dd}
Generative Adversarial Networks (GAN)~\cite{goodfellow2014generative}, conditional GAN~\cite{mirza2014conditional} and DCGAN \cite{radford2015unsupervised} learns to synthesize real looking images.
Though they are related, our goal is not to produce real looking samples but a small set of condensed samples that are aimed to train models.
The most related work to ours is Dataset Distillation~(DD)~\cite{wang2018dataset} that also aims to generate a small set of informative training samples.
To this end, the authors consider the network parameters as a function of synthetic data and learn them by minimizing the training loss over the real data in terms of the synthetic data. 
This idea is further extended to text dataset distillation in \cite{sucholutsky2019soft}. 
Unlike \cite{wang2018dataset}, our model aims to obtain not only similar generalization performance with a model trained on the real data but also similar solution in the parameter space by matching the gradients.
As a result, our method is scalable to large models and the generated images are not architecture dependent, \ie they can be used to train various deep network architectures.
In \cref{sec.exp}, we also compare to \cite{wang2018dataset} and show that our method outperforms it with a wide margin in multiple benchmarks.




\paragraph{Knowledge distillation.}
Our method is also related to knowledge distillation~(KD)~\cite{hinton2015distilling} based techniques~\cite{bucilua2006model,ba2014deep,romero2014fitnets} that transfer the knowledge from an ensemble of models to a single one.
Though our method can also be seen as KD from a teacher to a student network, we use the knowledge distillation to learn synthesizing training images.
In addition, our model does not require different teacher and student networks as in \cite{hinton2015distilling} and can work with identical teacher-student models.
Recent zero-shot KD methods~\cite{dfkd-nips-lld-17,zskd-icml-2019} aims to perform KD from a trained model in the absence of training data by generating synthetic data as the intermediate production to further use.
Though these methods also train student models using only synthetic samples, they require pretrained teacher models to provide the knowledge, \ie to obtain the features and labels.
Unlike \cite{dfkd-nips-lld-17,zskd-icml-2019}, our method distills knowledge from data but not from pretrained models.


\paragraph{Understanding deep image representations.} 
Our method is also related to the methods~\cite{zeiler2014visualizing,mahendran2015understanding,zhu2019deep} that project the feature activations back to the input pixel space \cite{zeiler2014visualizing}, reconstruct the input image by matching the feature activations~\cite{mahendran2015understanding}, recover private training images for given training gradients.
Unlike \cite{zeiler2014visualizing,mahendran2015understanding,zhu2019deep}, our goal is not to recover the original training images but to synthesize a set of condensed training images.

 


==> table_fsda.tex <==
\centering
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{cccccccc}
\toprule
                                  & I/C             & Random              & Herding         & K-Center       & Forgetting      &   Ours  &  No Adapt           \\ \midrule
\multirow{2}{*}{S$\rightarrow$M}    & 1     & 75.7$\pm$4.5  & 93.5$\pm$0.8  & 93.1$\pm$1.1  & 41.5$\pm$6.4     & \bf{94.4$\pm$0.4}  & \multirow{2}{*}{76.5$\pm$1.7} \\
                                    & 10    & 97.0$\pm$0.5  & 95.8$\pm$0.4  & 90.8$\pm$0.7  & 74.8$\pm$1.8     & \bf{97.7$\pm$0.2}   &  \\ \midrule
\multirow{2}{*}{M$\rightarrow$S}    & 1     & 17.2$\pm$2.2  & 25.0$\pm$3.2  & 25.0$\pm$3.2  & 12.8$\pm$1.4     & \bf{35.7$\pm$2.1} & \multirow{2}{*}{31.0$\pm$1.2} \\ 
                                    & 10    & 56.1$\pm$1.8  & 61.7$\pm$2.1  & 19.0$\pm$1.6  & 32.3$\pm$2.2     & \bf{74.8$\pm$0.8}   &           \\ \bottomrule
\end{tabular}



==> table_runtime.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{cccccc}
\toprule
                           &                            & MNIST             & FashionMNIST      & SVHN              & CIFAR10 \\ 
\midrule
\multirow{3}{*}{Images}             & Whole Dataset     & 60000  & 60000  & 73257  & 50000        \\ 
                           & Ours 1 img/cls             & 10     & 10     & 10     & 10        \\ 
                           & Ours 10 img/cls            & 100    & 100    & 100    & 100        \\ \midrule
\multirow{3}{*}{Time (s)}  & Whole Dataset          & 773               & 776               & 931               & 644        \\ 
                           & Ours 1 img/cls             & 0.6           & 0.6               & 0.6               & 0.6        \\ 
                           & Ours 10 img/cls            & 1.3           & 1.3               & 1.3               & 1.3        \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{\footnotesize{Training time for a randomly initialized ConvNet on whole dataset and our condensed set.}}
\label{tab:time}
\end{table}




==> table_soa_dd.tex <==

\begin{table}
\centering
\scriptsize
\setlength{\tabcolsep}{4pt}
\begin{tabular}{cccccccccc}
\hline
\multirow{2}{*}{}           & \multirow{2}{*}{Img/Cls} & \multirow{2}{*}{Ratio \%} & \multicolumn{4}{c}{Core-set Selection}   & \multicolumn{2}{c}{Synthetic Data} & \multirow{2}{*}{Whole Dataset} \\ \cline{4-9}
                    &       &              & Random          & Herding         & K-Center       & Forgetting      & DD           & Ours &             \\ \hline
\multirow{2}{*}{MNIST}      & 1   & 0.017  & 56.7$\pm$9.7  & 73.2$\pm$7.7  & 71.7$\pm$8.6  & 25.7$\pm$4.7  & -              & \textbf{85.0$\pm$1.6} & \multirow{2}{*}{99.5$\pm$0.0} \\ \cline{2-9} 
                            & 10  & 0.17   & 91.2$\pm$1.3  & 84.6$\pm$2.2  & 78.4$\pm$2.6  & 61.6$\pm$4.5  & 79.5$\pm$8.1   & \textbf{93.4$\pm$0.6} &  \\ \cline{1-10} 
\multirow{2}{*}{CIFAR10}    & 1   & 0.02   & 16.4$\pm$2.3  & 15.7$\pm$1.8  & 15.7$\pm$1.7  & 13.6$\pm$2.0  & -              & \textbf{24.2$\pm$0.9} & \multirow{2}{*}{83.1$\pm$0.2}          \\ \cline{2-9} 
                            & 10  & 0.2    & 26.4$\pm$0.8  & 28.7$\pm$0.8  & 20.9$\pm$1.1  & 20.9$\pm$1.4  & 36.8$\pm$1.2   & \textbf{39.1$\pm$1.2} &           \\ \cline{1-10} 
\end{tabular}
\caption{The performance ($\%$) comparison to Dataset Distillation (DD) method \cite{wang2018dataset}. 
For fair comparison, we use the same architectures (LeNet for MNIST and AlexCifarNet for CIFAR10) as that presented in \cite{wang2018dataset}, where AlexCifarNet is the customized AlexNet. Img/Cls denotes the number of images per class.}
\label{tab:sota_dd}
\end{table}



